TransAct: Transformer-based Realtime User Action Model for Recommendation at Pinterest

Sequential models that encode user activity for next action prediction have become a popular design choice for building web-scale personalized recommendation systems. Traditional methods of sequential recommendation either utilize end-to-end learning on realtime user actions, or learn user representations separately in an offline batch-generated manner. This paper (1) presents Pinterest's ranking architecture for Homefeed, our personalized recommendation product and the largest engagement surface; (2) proposes TransAct, a sequential model that extracts users' short-term preferences from their realtime activities; (3) describes our hybrid approach to ranking, which combines end-to-end sequential modeling via TransAct with batch-generated user embeddings. The hybrid approach allows us to combine the advantages of responsiveness from learning directly on realtime user activity with the cost-effectiveness of batch user representations learned over a longer time period. We describe the results of ablation studies, the challenges we faced during productionization, and the outcome of an online A/B experiment, which validates the effectiveness of our hybrid ranking model. We further demonstrate the effectiveness of TransAct on other surfaces such as contextual recommendations and search. Our model has been deployed to production in Homefeed, Related Pins, Notifications, and Search at Pinterest.

==> sections/i.tex <==
\section{Introduction}

% Why’s rec sys important
The proliferation of online content in recent years has created an overwhelming amount of information for users to navigate. 
To address this issue, recommender systems are employed  in various industries to help users find relevant items from a vast selection, including products, images, videos, and music. 
% , making it easier for them to find what they want. 
By providing personalized recommendations, businesses and organizations can better serve their users and keep them engaged with the platform. 
Therefore, recommender systems are vital for businesses as they drive growth by boosting engagement, sales and revenue.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.85\linewidth]{figures/Homefeed_web_square.png}
  % \caption{Illustration of generating Pinterest Homefeed page using a 3-stage RS}
  \caption{Pinterest Homefeed Page}
  \label{fig:hf}
  \Description{Pinterest Homefeed page}
\end{figure}

% Background of PINS Homefeed ranking. Previous PINS work (PinSage, Pinnerformer)
As one of the largest content sharing and social media platforms, Pinterest hosts billions of pins with rich contextual and visual information, and brings inspiration to over 400 million users. 
Upon visiting Pinterest, users are immediately presented with the Homefeed page as shown in Figure~\ref{fig:hf}, which serves as the primary source of inspiration and accounts for the majority of overall user engagement on the platform.
The Homefeed page is powered by a 3-stage recommender system that retrieves, ranks, and blends content based on user interests and activities. 
At the retrieval stage, we filter billions of pins created on Pinterest to thousands, based on a variety of factors such as user interests, followed boards, etc. Then we use a pointwise ranking model to rank candidate pins by predicting their personalized relevance to users. 
Finally, the ranked result is adjusted using a blending layer to meet business requirements.

% We focus on the ranking stage in this paper. 
% To help the ranking task, we have built pre-trained item or user embeddings, which uses a reasonable amount of space to represent rich information. Some successful methods include Pinnerformer~\cite{pinnerformer}, PinSage~\cite{PinSage}, itemsage~\cite{itemsage}, etc.



% Existing work for realtime ranking
Realtime recommendation is crucial because it provides a quick and up-to-date recommendation to users, improving their overall experience and satisfaction. 
The integration of realtime data, such as recent user actions, results in more accurate recommendations. This, in turn, increases the probability of users discovering relevant items. 
Research in this area typically focuses on reducing the complexity of the system\cite{chatzopoulos2016readme}, handling high-velocity data streams\cite{6542425}, and dealing with dynamic changes in user behavior~\cite{grbovic2018real, 10.1145/2699670}. 

% Hybrid of Pinnerformer (batch)(larger model) + TransAct (realtime)
Previous research has shown that user embeddings, such as those generated by PinnerFormer~\cite{pinnerformer}, can effectively represent long-term user interests based on past actions over an extended time frame. However, realtime inference of these methods can be computationally expensive and complex.
As a result, user embedding features are often generated as \textit{batch} features (e.g. generated daily), which are cost-effective to serve across multiple applications
However, batch features have limitations in promptly capturing users' changing interests and they are not trained end-to-end with the objectives of the target application.
To address these limitations, we propose realtime-batch hybrid ranking, which incorporates both \textit{realtime} user action sequence signals and \textit{batch} user embeddings. 
We develop a transformer-based realtime user action model (TransAct) to encode realtime user action sequence signals and learn users' short term interests. 
% TransAct is trained end-to-end with the objectives of the RS.
By combining both batch features and realtime features, the hybrid ranking model offers users realtime feedback on their recent actions, while also accounting for their long-term interests. This leads to an overall improvement in the user experience on the Homefeed page.

% Limitation of previous sequential recommendation/ novelty

Sequential recommendation systems use a user's action history as input and apply recommendation algorithms to suggest appropriate items. Recent work~\cite{donkers2017sequential, hidasi2015session, tan2016improved, zhou2019deep, tang2018personalized, tuan20173d} has been using deep learning techniques, such as recurrent neural networks (RNNs)~\cite{rnn} and convolutional neural networks (CNNs)~\cite{cnn}, to process users' action history. Some studies~\cite{DIN, zhang2019next, alibaba_seq_tfmr, li2020time, SASRec, sun2019bert4rec} have also adopted the attention mechanism~\cite{tfmr} to model user action sequence features. 
In this work, we also employ the self-attention mechanism for realtime user sequence modeling for its superior capability in encoding sequential inputs. 
% One limitation of the existing sequential recommendation is that they
To the best of our knowledge, this is the first method that builds a realtime-batch hybrid ranking model which uses users' action sequences in both realtime and batch settings. 
For the realtime user actions, we propose TransAct, a novel transformer-based module to encode users' short-term interests.
For non-realtime user actions, we encode it into a batch user representation\cite{pinnerformer}. 
We provide an in-depth analysis of the challenges posed by utilizing real-time user sequence features, such as the potential decrease in recommendation diversity and engagement decay.



The major contributions of this paper are summarized as follows:
\begin{itemize}
\item We describe the architecture of production ranking system at Pinterest. We propose TransAct on top of the current ranking model, which effectively learns users' short-term interests from their most recent actions. With TransAct as the realtime component, we build a realtime-batch hybrid ranking model and improve the performance greatly.
\item We provide details on the serving optimization of TransAct. We ran into scalability issues with our model serving infrastructure and need to transition to GPU serving. We provide some optimizations that we have done to make GPU serving for Pinnability with TransAct effective.
\item We conduct a comprehensive ablation study to thoroughly examine various design choices, which provides valuable insights of the system's functionality.
\item We conduct online A/B experiments on a real-world recommendation system using TransAct. We demonstrate some practical issues in the online environment, such as recommendation diversity drop and engagement decay. We propose solutions to address these issues.  
% \item Our model has been deployed as the Homefeed ranking model of Pinterest, one of the largest content sharing and social media platforms. As a result, it boosts the Homefeed repin\footnote{A "repin" on Pinterest refers to the action of saving an existing pin to another board by a user.} volume by 11\%.

\end{itemize}

% Structure of the paper
% \td{check}
The remainder of this paper is organized as follows: Related
work is reviewed in Section~\ref{sec:related_work}. Section~\ref{sec:method} describes the design of TransAct and the details of bringing it to production. Experiment results are reported in Section~\ref{sec:exp}. We discuss some findings beyond experiments in Section~\ref{sec:discussion}. Finally, we conclude our work in Section~\ref{sec:conclusion}.
% Learnings









% \begin{itemize}
% \item Hybrid setup
% \item Ablation study: Using both positive and negative actions, Early fusion with candidate pin
% \item Diversity: time window mask
% \item Frequent retraining
% \item is good for cold-start users (non-core)
% \end{itemize}


% 1. Hybrid setup
% w. No extensive ablation study on the model architecture Model: early fusion, random time window.
% Did not discuss practical challenge: latency, GPU serving
% Ali’s Search based user seq does have practical challenge
% id feature only (but we don’t have img_sig feature)	
% 3. Diversity


% Most existing recommender systems use a wide and deep architecture, where the inputs are user features, item features and context features. The model usually learns the relevance score between the user and item over a given context. The traditional way to get user or item features are mostly through feature engineering. And then the model use the hand-picked features to predict the relevance between user and items. Raw features are usually very limited in the amount of information that they can represent. More advanced techniques include learning pre-trained item or user embedding, where it can use a reasonable amount of space to represent richer information. Some successful pre-trained embeddings are Pinnerformer\cite{pinnerformer}, itemsage\cite{itemsage}, etc. However, one of the major shortcomings of pre-trained embedding is that they are usually expensive to infer in realtime due to their high computational cost and infra complexity. 
